In-Context Learning User Simulators for Task-Oriented Dialog Systems

This paper presents a novel application of large language models in user simulation for task-oriented dialog systems, specifically focusing on an in-context learning approach. By harnessing the power of these models, the proposed approach generates diverse utterances based on user goals and limited dialog examples. Unlike traditional simulators, this method eliminates the need for labor-intensive rule definition or extensive annotated data, making it more efficient and accessible. Additionally, an error analysis of the interaction between the user simulator and dialog system uncovers common mistakes, providing valuable insights into areas that require improvement. Our implementation is available at https://github.com/telepathylabsai/prompt-based-user-simulator.

==> tables/prompt_april_27.tex <==
\begin{table*}[ht]
\centering\small
\begin{tabular}{p{0.2in}p{0.4in}|ccccc}
\# shots & bullet point requirements &  \multicolumn{5}{c}{Task Descriptions} \\
\hline
& & default & default + domains & extra personality & minimal & none \\
\hline

0 & FALSE & 0.40 (0.08, 0.68) & 0.41 (0.07, 0.68) & 0.49 ( \textbf{0.15}, 0.65) & 0.24 (0.01, 0.71) & 0.42 (0.07, 0.64) \\
1 & FALSE & 0.51 (0.10, 0.67) & 0.51 (0.10, 0.66) & \textbf{0.54} (0.12, 0.62) & 0.41 (0.05, 0.70) & 0.46 (0.06, 0.65) \\
 & TRUE & 0.49 (0.08, 0.69) &  &  &  &  \\
2 & FALSE & 0.51 (0.12, 0.66) & \textbf{0.51} (0.10, 0.67) & 0.51 (0.11, 0.62) & \textbf{0.44 (0.10, 0.69)} & 0.47 (0.07, 0.63) \\
 & TRUE & 0.51 (0.11, 0.68) &  &  &  &  \\
3 & FALSE & 0.51 (\textbf{0.14}, 0.67) & 0.50 (\textbf{0.15}, 0.66) & 0.53 (0.13, 0.61) & 0.41 (0.07, 0.69) & 0.47 (0.09, 0.66) \\
 & TRUE & 0.50 (0.12, 0.68) &  &  &  &  \\

\hline
4 & FALSE & \textbf{0.53} (0.13, 0.66) &  &  &  & \textbf{0.48} (0.09, 0.65) \\
5 & FALSE & 0.51 (0.12, 0.66) &  &  &  &  0.45 ( \textbf{0.10}, 0.66) \\
6 & FALSE & 0.53 (0.11, 0.65) &  &  &  & 0.46 (0.08, 0.65) \\
%8 & FALSE & 0.50 (0.12, 0.66) &  &  &  &  
\end{tabular}
\caption{Prompt engineering results after running 200 identical conversations under varying number of shots/examples, requirements representation (structured bullet points vs descriptive), and 5 task description flavors. Reported scores are slot fulfillment rate (dialog success ratio, MSTTR). In 0-shot setting, default + domains prompt is the same as default, since domains are derived from shots's domains. All models run with FLAN-T5.}
\label{tab:prompt}
\end{table*}

==> tables/prompt_nk_april_22.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{ccccc}
\multirow{2}{*}{\# shots} & \multirow{2}{*}{bullet pointed goal} & \multicolumn{3}{c}{task description} \\
                          &                                      & 1          & 2          & 3          \\
\hline
0                         & False                                & 0.16(0.02)       & 0.18(0.08)       & 0.31(0.1)       \\
\hline
\multirow{2}{*}{1}        & True                                 & 0.30(0.16)       & 0.39(0.18)       & 0.35(0.12)       \\
                          & False                                & 0.35(0.10)       & 0.27(0.14)       & 0.36(0.12)        \\
\hline
\multirow{2}{*}{2}        & True                                 & 0.38(0.12)       & 0.36(0.12)       & 0.33(0.12)        \\
                          & False                                & 0.31(0.12)       & 0.28(0.08)       & 0.27(0.12)        \\
\hline
\multirow{2}{*}{3}        & True                                 & 0.30(0.14)       & 0.35(0.12)       & 0.28(0.06)        \\
                          & False                                & 0.27(0.14)       & 0.31(0.16)       & 0.41(0.18)        
\end{tabular}
\caption{F1 scores (and success number of dialogs) achieved with google/flanT5-xl with different strategies of prompt.}
\end{table*}
